Statistical models for cores decomposition of an undirected random graph

The $k$-core decomposition is a widely studied summary statistic that describes a graph's global connectivity structure. In this paper, we move beyond using $k$-core decomposition as a tool to summarize a graph and propose using $k$-core decomposition as a tool to model random graphs. We propose using the shell distribution vector, a way of summarizing the decomposition, as a sufficient statistic for a family of exponential random graph models. We study the properties and behavior of the model family, implement a Markov chain Monte Carlo algorithm for simulating graphs from the model, implement a direct sampler from the set of graphs with a given shell distribution, and explore the sampling distributions of some of the commonly used complementary statistics as good candidates for heuristic model fitting. These algorithms provide first fundamental steps necessary for solving the following problems: parameter estimation in this ERGM, extending the model to its Bayesian relative, and developing a rigorous methodology for testing goodness of fit of the model and model selection. The methods are applied to a synthetic network as well as the well-known Sampson monks dataset.

==> degeneracy.tex <==
Here I am attempting to add points on what is missing- in the paper
\begin{enumerate}
	\item Discussion on the support restriction of the model and why it is important. How it avoids the problem of the ERGM being a mixture of complete and empty graph. The $\leq m $ assumption still makes it a mixture of the empty and the most complete graph, but the $=m$ assumption avoids this. Say that this can or should be done for other ERGMS. Real networks are sparse, does not make sense to have statistical models that put mass on very dense graphs or complete graphs. Also, as Despina suggested, it is making the normalizing constant simpler in the sense that we have lesser number of graphs to count.
	\item Add a more detailed discussion on how it is different from the $\beta$ model. Show it by example! May be put it as a proposition!
	\item Add a more detailed discussion on the asymptotics of the polytope of the restricted model. As $n$ grows and $m$ remains fixed, more and more points appear in the polytope and it is better! Show this by figures!
	
\end{enumerate}

State this as a theorem:

If you have more than one ``community'' in a graph, the degeneracy is bounded. 

What I want to formalize is the following idea - If you have a complete graph, everybody is connected to everybody. There is only one community. Everybody can communicate with everyone directly. But lets say there are two ``communities'' (Using whatever definition of communities you like). Then this means that there exist more edges 


